Mitigating subjectivity and bias in AI development indices: A robust approach to redefining country rankings

Countries worldwide have been implementing different actions national strategies for Artificial Intelligence (AI) to shape policy priorities and guide their development concerning AI. Several AI indices have emerged to assess countries' progress in AI development, aiding decision-making on investments and policy choices. Typically, these indices combine multiple indicators using linear additive methods such as weighted sums, although they are limited in their ability to account for interactions among indicators. Another limitation concerns the use of deterministic weights, which can be perceived as subjective and vulnerable to debate and scrutiny, especially by nations that feel disadvantaged. Aiming at mitigating these problems, we conduct a methodological analysis to derive AI indices based on multiple criteria decision analysis. Initially, we assess correlations between different AI dimensions and employ the Choquet integral to model them. Thus, we apply the Stochastic Multicriteria Acceptability Analysis (SMAA) to conduct a sensitivity analysis using both weighted sum and Choquet integral in order to evaluate the stability of the indices with regard the weights. Finally, we introduce a novel ranking methodology based on SMAA, which considers several sets of weights to derive the ranking of countries. As a result, instead of using predefined weights, in the proposed approach, the ranking is achieved based on the probabilities of countries in occupying a specific position. In the computational analysis, we utilize the data employed in The Global AI Index proposed by Tortoise. Results reveal correlations in the data, and our approach effectively mitigates bias. In the sensitivity analysis, we scrutinize changes in the ranking resulting from weight adjustments. We demonstrate that our proposal rankings closely align with those derived from weight variations, proving to be more robust.

==> tab_ranking_tortoise.tex <==
\begin{tabular}{ll}
\toprule
Position &       Country \\
\midrule
1 &      USA \\
2 &    China \\
3 &       UK \\
4 &   Canada \\
5 &   Israel \\
6 &    Sing. \\
7 &       SK \\
8 &       NL \\
9 &  Germany \\
\bottomrule
\end{tabular}

==> tab_ws_ranking_paises_pesos_ordenados.tex <==
\begin{tabular}{ll}
\toprule
Position&       Country \\
\midrule
1 &      USA \\
2 &    China \\
3 &       UK \\
4 &   Israel \\
5 &    Sing. \\
6 &   Canada \\
7 &  Germany \\
8 &       NL \\
9 &       SK \\
\bottomrule
\end{tabular}





\begin{comment}


\begin{tabular}{ll}
\toprule
{} &                         Paises \\
\midrule
1  &  United States of America \\
2  &                     China \\
3  &            United Kingdom \\
4  &                 Singapore \\
5  &                    Canada \\
6  &                    Israel \\
7  &                   Germany \\
8  &           The Netherlands \\
9  &               South Korea \\
10 &                   Ireland \\
11 &                    France \\
12 &                   Denmark \\
13 &                     Japan \\
14 &                     India \\
15 &                    Sweden \\
16 &                 Hong Kong \\
17 &                   Finland \\
18 &                 Australia \\
19 &                Luxembourg \\
20 &               Switzerland \\
21 &                    Norway \\
22 &                   Austria \\
23 &                   Estonia \\
24 &                    Taiwan \\
25 &                     Spain \\
26 &                    Russia \\
27 &              Saudi Arabia \\
28 &               New Zealand \\
29 &                  Slovenia \\
30 &                   Belgium \\
31 &                    Poland \\
32 &                     Malta \\
33 &      United Arab Emirates \\
34 &                   Iceland \\
35 &                  Portugal \\
36 &            Czech Republic \\
37 &                     Italy \\
38 &                 Lithuania \\
39 &                    Brazil \\
40 &                    Greece \\
41 &                  Malaysia \\
42 &                  Slovakia \\
43 &                   Hungary \\
44 &                    Turkey \\
45 &                    Mexico \\
46 &                     Qatar \\
47 &                 Argentina \\
48 &                     Chile \\
49 &                   Uruguay \\
50 &                  Colombia \\
51 &                   Bahrain \\
52 &                   Vietnam \\
53 &                 Indonesia \\
54 &                   Tunisia \\
55 &              South Africa \\
56 &                   Armenia \\
57 &                   Morocco \\
58 &                 Sri Lanka \\
59 &                     Egypt \\
60 &                     Kenya \\
61 &                  Pakistan \\
62 &                   Nigeria \\
\bottomrule
\end{tabular}

\end{comment}

==> tab_ws_ranking_paises_pesos_sem_ordem.tex <==
\begin{tabular}{ll}
\toprule
Position&       Country \\
\midrule
1 &      USA \\
2 &    China \\
3 &   Canada \\
4 &       SK \\
5 &       UK \\
6 &       NL \\
7 &   France \\
8 &  Germany \\
9 &    Sing. \\
\bottomrule
\end{tabular}













\begin{comment}


\begin{tabular}{ll}
\toprule
Position &                         Country \\
\midrule
1  &  United States of America \\
2  &                     China \\
3  &                    Israel \\
4  &            United Kingdom \\
5  &                    France \\
6  &                   Germany \\
7  &                    Canada \\
8  &                 Singapore \\
9  &           The Netherlands \\
10 &               South Korea \\
11 &                 Australia \\
12 &                   Ireland \\
13 &                   Finland \\
14 &                Luxembourg \\
15 &                     Japan \\
16 &                     India \\
17 &                   Estonia \\
18 &      United Arab Emirates \\
19 &                    Taiwan \\
20 &                    Poland \\
21 &               Switzerland \\
22 &                   Austria \\
23 &                     Spain \\
24 &                  Slovenia \\
25 &                  Portugal \\
26 &                   Denmark \\
27 &              Saudi Arabia \\
28 &                    Sweden \\
29 &                 Hong Kong \\
30 &               New Zealand \\
31 &                   Belgium \\
32 &                     Italy \\
33 &                    Russia \\
34 &                    Norway \\
35 &                     Malta \\
36 &            Czech Republic \\
37 &                    Turkey \\
38 &                   Iceland \\
39 &                 Lithuania \\
40 &                 Argentina \\
41 &                  Slovakia \\
42 &                    Brazil \\
43 &                  Malaysia \\
44 &                    Greece \\
45 &                     Chile \\
46 &                    Mexico \\
47 &                  Colombia \\
48 &                     Qatar \\
49 &                   Hungary \\
50 &                   Uruguay \\
51 &                 Indonesia \\
52 &                   Bahrain \\
53 &                   Vietnam \\
54 &                   Tunisia \\
55 &                   Morocco \\
56 &              South Africa \\
57 &                   Armenia \\
58 &                 Sri Lanka \\
59 &                     Egypt \\
60 &                     Kenya \\
61 &                   Nigeria \\
62 &                  Pakistan \\
\bottomrule
\end{tabular}

\end{comment}

==> tab_ws_winning_pesos_ordenados.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &      0 &      1 &      2 &      3 &      4 &      5 &      6 &      7 \\
\midrule
0 &  100.0 &    0.0 &    0.0 &   0.00 &   0.00 &   0.00 &   0.00 &   0.00 \\
1 &    0.0 &  100.0 &    0.0 &   0.00 &   0.00 &   0.00 &   0.00 &   0.00 \\
2 &    0.0 &    0.0 &  100.0 &   0.00 &   0.00 &   0.00 &   0.00 &   0.00 \\
3 &    0.0 &    0.0 &    0.0 &   1.89 &  46.53 &  41.87 &   9.64 &   0.06 \\
4 &    0.0 &    0.0 &    0.0 &  90.01 &   8.79 &   0.93 &   0.27 &   0.00 \\
5 &    0.0 &    0.0 &    0.0 &   1.32 &   2.47 &   4.83 &  42.64 &  26.93 \\
6 &    0.0 &    0.0 &    0.0 &   6.15 &   7.20 &   7.57 &  22.29 &  24.29 \\
7 &    0.0 &    0.0 &    0.0 &   0.58 &  34.19 &  43.85 &  20.27 &   1.09 \\
\bottomrule
\end{tabular}




==> tab_ws_winning_pesos_sem_ordem.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &      0 &      1 &      2 &      3 &      4 &      5 &      6 &     7 \\
\midrule
0 &  99.31 &   0.65 &   0.01 &   0.01 &   0.01 &   0.01 &   0.00 &  0.00 \\
1 &   0.69 &  93.47 &   2.69 &   1.07 &   0.75 &   0.67 &   0.49 &  0.06 \\
2 &   0.00 &   2.63 &  58.16 &  28.03 &   3.86 &   3.80 &   1.49 &  0.77 \\
3 &   0.00 &   0.00 &   0.03 &   9.57 &  16.60 &  20.34 &  22.53 &  9.83 \\
4 &   0.00 &   0.00 &   2.77 &  13.68 &  24.89 &  25.56 &  17.70 &  9.65 \\
5 &   0.00 &   0.00 &  29.44 &  21.38 &   8.91 &   8.50 &  13.83 &  8.43 \\
6 &   0.00 &   0.01 &   1.19 &   4.49 &   4.74 &   2.75 &   2.98 &  5.18 \\
7 &   0.00 &   0.53 &   3.58 &  15.23 &  26.67 &  23.30 &  17.47 &  8.84 \\
\bottomrule
\end{tabular}


